Abstracting Effect Systems for Algebraic Effect Handlers

Many effect systems for algebraic effect handlers are designed to guarantee that all invoked effects are handled adequately. However, respective researchers have developed their own effect systems that differ in how to represent the collections of effects that may happen. This situation results in blurring what is required for the representation and manipulation of effect collections in a safe effect system. In this work, we present a language ${\lambda_{\mathrm{EA}}}$ equipped with an effect system that abstracts the existing effect systems for algebraic effect handlers. The effect system of ${\lambda_{\mathrm{EA}}}$ is parameterized over effect algebras, which abstract the representation and manipulation of effect collections in safe effect systems. We prove the type-and-effect safety of ${\lambda_{\mathrm{EA}}}$ by assuming that a given effect algebra meets certain properties called safety conditions. As a result, we can obtain the safety properties of a concrete effect system by proving that an effect algebra corresponding to the concrete system meets the safety conditions. We also show that effect algebras meeting the safety conditions are expressive enough to accommodate some existing effect systems, each of which represents effect collections in a different style. Our framework can also differentiate the safety aspects of the effect collections of the existing effect systems. To this end, we extend ${\lambda_{\mathrm{EA}}}$ and the safety conditions to lift coercions and type-erasure semantics, propose other effect algebras including ones for which no effect system has been studied in the literature, and compare which effect algebra is safe and which is not for the extensions.

==> macro.tex <==
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

\setlist{topsep=0pt}
\setlist[enumerate]{label=(\arabic*), ref=(\arabic*)}

\def\divcase#1{\textit{Case} #1:}
\newlist{divcases}{description}{5}
\setlist[divcases]{format=\divcase}

\newcommand{\defeq}{\stackrel{\rm \tiny def}{=}}

\newcommand{\rname}[2]{\textnormal{\scshape #1\_#2}}

\newcommand{\imply}{\text{ implies }}
\newcommand{\tand}{\text{ and }}
\newcommand{\tor}{\text{ or }}
\newcommand{\tif}{\text{if }}
\newcommand{\twhere}{\text{where }}
\newcommand{\tquad}{\hspace{1em}}
\newcommand{\tqquad}{\hspace{2em}}

\newcommand{\ari}{\mathrm{ConsSig}}
\newcommand{\labels}{\mathrm{dom}(\Slabel)}
\newcommand{\labari}{\mathrm{LabSig}}
\newcommand{\FS}{\mathit{FS}}
\newcommand{\EC}{\mathrm{dom}(\Sbase)}
\newcommand{\lift}[1]{(#1)^{\uparrow}}
\newcommand{\Sbase}{\Sigma_{\mathrm{eff}}}
\newcommand{\Slabel}{\Sigma_{\mathrm{lab}}}
\newcommand{\Gbase}{\Gamma_{\mathrm{base}}}
\newcommand{\Terms}[2][\Gbase]{\mathit{Terms}^{#2}(\Sbase, #1)}
\newcommand{\carry}[1]{\mathit{Crr}^{#1}}
\newcommand{\interp}[1]{(#1)^{*}}
\newcommand{\dbra}[2][\eta]{\llbracket #2 \rrbracket_{#1}}

\newcommand{\ECSet}{\EC_\mathrm{Set}}
\newcommand{\SbaseSet}{\Sbase^\mathrm{Set}}
\newcommand{\SbaseMSet}{\Sbase^\mathrm{MSet}}
\newcommand{\SbaseRow}{\Sbase^\mathrm{Row}}

\newcommand{\typelikes}{\mathit{Typelikes}}
\newcommand{\typvar}{\mathit{TypVar}}
\newcommand{\labvar}{\mathit{LabVar}}
\newcommand{\effvar}{\mathit{EffVar}}
\newcommand{\tvar}{\mathit{TVar}}

\newcommand{\dom}{\mathrm{dom}}
\newcommand{\ftv}{\mathrm{FTV}}
\newcommand{\List}{\mathit{List}}

\newcommand{\app}[2]{#1\,#2}
\newcommand{\funsym}{\mathit{FuncSymbol}}
\newcommand{\effdecl}[1]{\mathbf{effect} \ {#1}}
\newcommand{\letdecl}[1]{\mathbf{let} \ {#1} =}
\newcommand{\namecollect}{\mathit{accumulate}}

\newcommand{\eff}{\mathit{Eff}}

\newcommand{\eanameSet}{\ensuremath{\mathrm{Set}}}
\newcommand{\eanameEraseSet}{\ensuremath{\mathrm{ESet}}}
\newcommand{\eanameSimpleRow}{\ensuremath{\mathrm{SimpR}}}
\newcommand{\eanameEraseSimpleRow}{\ensuremath{\mathrm{ESimpR}}}
\newcommand{\eanameScopedRow}{\ensuremath{\mathrm{ScpR}}}
\newcommand{\eanameEraseScopedRow}{\ensuremath{\mathrm{EScpR}}}
\newcommand{\eanameMSet}{\ensuremath{\mathrm{MSet}}}
\newcommand{\eanameEraseMSet}{\ensuremath{\mathrm{EMSet}}}

\newcommand{\eaSet}{\ensuremath{\mathrm{EA_{\eanameSet}}}}
\newcommand{\eaEraseSet}{\ensuremath{\mathrm{EA_{\eanameEraseSet}}}}
\newcommand{\eaSimpleRow}{\ensuremath{\mathrm{EA_{\eanameSimpleRow}}}}
\newcommand{\eaEraseSimpleRow}{\ensuremath{\mathrm{EA_{\eanameEraseSimpleRow}}}}
\newcommand{\eaScopedRow}{\ensuremath{\mathrm{EA_{\eanameScopedRow}}}}
\newcommand{\eaEraseScopedRow}{\ensuremath{\mathrm{EA_{\eanameEraseScopedRow}}}}
\newcommand{\eaMSet}{\ensuremath{\mathrm{EA_{\eanameMSet}}}}
\newcommand{\eaEraseMSet}{\ensuremath{\mathrm{EA_{\eanameEraseMSet}}}}

\newcommand{\pretnars}{\textnormal{\scshape Eff}}
\newcommand{\links}{\textnormal{\scshape Links}}
\newcommand{\koka}{\textnormal{\scshape Koka}}
\newcommand{\trans}[1]{\ensuremath{\mathbb{T}_{#1}}}

\newcommand{\lang}{\ensuremath{\lambda_{\mathrm{EA}}}}

\newcommand{\draftcomment}[2]{\ifdraft{\phantom{}\color{#1}{#2}}\else\ifhmode\unskip\fi\fi}
\newcommand{\TY}[1]{\draftcomment{red}{TY: #1}}
\newcommand{\TS}[1]{\draftcomment{magenta}{TS: #1}}
\newcommand{\AI}[1]{\draftcomment{orange}{AI: #1}}
\newcommand{\OLD}[1]{\ifoldenable\draftcomment{cyan}{OLD: #1}\fi}
\newcommand{\OOLD}[1]{\ifoldenable\draftcomment{green}{OLD: #1}\fi}

\DeclareMathOperator{\cons}{::}
\DeclareMathOperator{\at}{@}

\definecolor{syntaxhighlight}{gray}{0.75}

\newcounter{safecondcounter}

\newcommand{\KSet}[2]{\ensuremath{#1(#2)}}
\newcommand{\EffSet}[1]{\KSet{ \mathbf{Eff} }{#1}}
\newcommand{\LabelSet}[1]{\KSet{ \mathbf{Lab} }{#1}}
\newcommand{\TypSet}[1]{\KSet{ \mathbf{Typ} }{#1}}

\newcommand{\bbZero}{\text{{\usefont{U}{DSSerif}{m}{n}0}}}

==> ott/core.tex <==
% generated by Ott 0.33 from: ott/core.ott
\newcommand{\ottdrule}[4][]{{\displaystyle\frac{\begin{array}{l}#2\end{array}}{#3}\quad\ottdrulename{#4}}}
\newcommand{\ottusedrule}[1]{\[#1\]}
\newcommand{\ottpremise}[1]{ #1 \\}
\newenvironment{ottdefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]}{}
\newenvironment{ottfundefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]\begin{displaymath}\begin{array}{l}}{\end{array}\end{displaymath}}
\newcommand{\ottfunclause}[2]{ #1 \equiv #2 \\}
\newcommand{\ottnt}[1]{\mathit{#1}}
\newcommand{\ottmv}[1]{\mathit{#1}}
\newcommand{\ottkw}[1]{\mathbf{#1}}
\newcommand{\ottsym}[1]{#1}
\newcommand{\ottcom}[1]{\text{#1}}
\newcommand{\ottdrulename}[1]{\textsc{#1}}
\newcommand{\ottcomplu}[5]{\overline{#1}^{\,#2\in #3 #4 #5}}
\newcommand{\ottcompu}[3]{\overline{#1}^{\,#2<#3}}
\newcommand{\ottcomp}[2]{\overline{#1}^{\,#2}}
\newcommand{\ottgrammartabular}[1]{\begin{supertabular}{llcllllll}#1\end{supertabular}}
\newcommand{\ottmetavartabular}[1]{\begin{supertabular}{ll}#1\end{supertabular}}
\newcommand{\ottrulehead}[3]{$#1$ & & $#2$ & & & \multicolumn{2}{l}{#3}}
\newcommand{\ottprodline}[6]{& & $#1$ & $#2$ & $#3 #4$ & $#5$ & $#6$}
\newcommand{\ottfirstprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottlongprodline}[2]{& & $#1$ & \multicolumn{4}{l}{$#2$}}
\newcommand{\ottfirstlongprodline}[2]{\ottlongprodline{#1}{#2}}
\newcommand{\ottbindspecprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottprodnewline}{\\}
\newcommand{\ottinterrule}{\\[5.0mm]}
\newcommand{\ottafterlastrule}{\\}
% \renewcommand{\ottnt}[1]{\mathsf{#1} }
\renewcommand{\ottkw}[1]{\mathbf{#1} }
\renewcommand{\ottcom}[1]{\textit{#1} }
\renewcommand{\ottcomplu}[5]{#1\mbox{}^{\,#2\in #3 #4 #5} }

\renewcommand{\ottdrulename}[1]{\textsc{#1} }

\newcommand{\ottmetavars}{
\ottmetavartabular{
 $ \ottmv{index} ,\, \ottmv{i} ,\, \ottmv{j} ,\, \ottmv{n} ,\, \ottmv{m} ,\, \ottmv{r} ,\, \ottmv{cont} $ & \ottcom{indices} \\
 $ \ottmv{integer} $ &  \\
 $ \ottmv{natvar} ,\, \mathit{n} ,\, \mathit{m} $ & \ottcom{natural numbers} \\
 $ \mathit{indexset} ,\, \mathit{I} ,\, \mathit{J} ,\, \mathit{N} $ &  \\
 $ \mathit{termvar} ,\, \mathit{x} ,\, \mathit{y} ,\, \mathit{z} ,\, \mathit{f} ,\, \mathit{g} ,\, \mathit{o} ,\, \mathit{p} ,\, \mathit{k} ,\, \mathit{xs} ,\, \mathit{ys} ,\, \_ ,\, \mathit{bad\_count\_f} ,\, \mathit{count\_f} $ &  \\
 $ \ottmv{typelikevar} ,\, \alpha ,\, \beta ,\, \gamma ,\, \tau ,\, \iota ,\, \rho $ &  \\
 $ \mathit{funcsymbol} ,\, \mathcal{F} ,\, \mathcal{C} $ &  \\
 $ \mathit{labelvar} ,\, \mathit{l} ,\, \mathsf{Exc} ,\, \mathsf{IO} ,\, \mathsf{Choice} ,\, \mathsf{Fail} ,\, \mathsf{State} ,\, \mathsf{Reader} ,\, \mathsf{Writer} ,\, \mathsf{Tick} ,\, \mathsf{Selection} $ &  \\
 $ \mathsf{opvar} ,\, \mathsf{op} ,\, \mathsf{raise} ,\, \mathsf{print} ,\, \mathsf{decide} ,\, \mathsf{fail} ,\, \mathsf{get} ,\, \mathsf{set} ,\, \mathsf{ask} ,\, \mathsf{tell} ,\, \mathsf{tick} ,\, \mathsf{select} $ &  \\
}}

\newcommand{\otte}{
\ottrulehead{\ottnt{e}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottnt{v}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{e_{{\mathrm{1}}}} \, \ottnt{e_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{v} \, S}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{v} \, \psi}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathbf{let} \, \mathit{x}  \ottsym{=}  \ottnt{e_{{\mathrm{1}}}} \, \mathbf{in} \, \ottnt{e_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottkw{effect} \, \Xi \, \mathbf{in} \, \ottnt{e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Handle} \, \ottnt{e} \, \mathbf{with} \, \ottnt{h}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \colorbox{syntaxhighlight}{$ \ottnt{e} $} } {\textsf{S}}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{e}  ] _{ \ottnt{label} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ [ \cdots [  \ottnt{e}  ] _{ \ottnt{label} } \cdots ]_{ \ottnt{label'} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\langle  c  \rangle  \ottnt{e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Handle} \, \ottnt{e} \, \mathbf{with} \, \ottnt{varh}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\llbracket  \ottnt{e}  \rrbracket}{}{}{}{}}

\newcommand{\ottv}{
\ottrulehead{\ottnt{v}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{x}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottkw{fun} \, \ottsym{(}  \mathit{g}  \ottsym{,}  \mathit{x}  \ottsym{,}  \ottnt{e}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  \alpha  \ottsym{:}  \ottnt{K}  \ottsym{.}  \ottnt{e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\psi  \Rightarrow  \ottnt{e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{OP}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{OP} \, \ottnt{Us}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{v} \, \ottnt{Subst}}{}{}{}{}}

\newcommand{\ottco}{
\ottrulehead{c}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \phantom{}\uparrow  \ottnt{label} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{label_{{\mathrm{1}}}}  \leftrightarrow  \ottnt{label_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{label}  :  c }{}{}{}{}\ottprodnewline
\ottprodline{|}{ c_{{\mathrm{1}}}  \cdot  c_{{\mathrm{2}}} }{}{}{}{}}

\newcommand{\ottconst}{
\ottrulehead{\ottnt{const}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottmv{integer}}{}{}{}{}}

\newcommand{\ottnum}{
\ottrulehead{\ottnt{num}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottmv{integer}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottmv{natvar}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{num_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{num_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ { c }_{ \ottnt{L} } ( \ottnt{num} ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{num}  \ottsym{)}} {\textsf{S}}{}{}{}}

\newcommand{\otth}{
\ottrulehead{\ottnt{h}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottsym{\{} \, \mathbf{return} \, \mathit{x}  \mapsto  \ottnt{e}  \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{}  \mathsf{op} \, \ottnt{Alphas} \, \mathit{p} \, \mathit{k}  \mapsto  \ottnt{e}  \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{}  \mathsf{op} \, \mathit{p} \, \mathit{k}  \mapsto  \ottnt{e}  \ottsym{\}}} {\textsf{S}}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{h} \, \ottnt{Subst}}{}{}{}{}}

\newcommand{\ottvarh}{
\ottrulehead{\ottnt{varh}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \{ \mathbf{return}\, x \mapsto  \ottnt{e_{\ottmv{r}}}  \}  \ottnt{upluses}  \{ ( \mathit{o}  :  \alpha   \Rightarrow   \beta )\, p\, k \mapsto  \ottnt{e}  \} }{}{}{}{}}

\newcommand{\otthClause}{
\ottrulehead{\ottnt{hClause}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathbf{return} \, \mathit{x}  \mapsto  \ottnt{e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathsf{op} \, \ottnt{Alphas} \, \mathit{p} \, \mathit{k}  \mapsto  \ottnt{e}}{}{}{}{}}

\newcommand{\ottupluses}{
\ottrulehead{\ottnt{upluses}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\uplus}{}{}{}{}\ottprodnewline
\ottprodline{|}{\uplus \, \cdots \, \uplus}{}{}{}{}}

\newcommand{\ottlabel}{
\ottrulehead{\ottnt{label}  ,\ \ottnt{L}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\iota}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{l}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{l} \, \ottnt{Us}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{label} } {\textsf{S}}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{-}} {\textsf{S}}{}{}{}}

\newcommand{\ottepsilon}{
\ottrulehead{\varepsilon}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\rho}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \bbZero }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \lift{ \ottnt{label} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathcal{F}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathcal{F} \, \ottnt{Us}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \varepsilon } {\textsf{S}}{}{}{}}

\newcommand{\ottrow}{
\ottrulehead{\varepsilon  ,\ {r}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\rho}{}{}{}{}\ottprodnewline
\ottprodline{|}{\langle  \rangle}{}{}{}{}\ottprodnewline
\ottprodline{|}{\langle  \ottnt{label}  \mid  \varepsilon  \rangle}{}{}{}{}\ottprodnewline
\ottprodline{|}{\langle  \ottnt{label_{{\mathrm{1}}}}  \mid  \langle  \cdots  \langle  \ottnt{label_{{\mathrm{2}}}}  \mid  \varepsilon  \rangle  \cdots  \rangle  \rangle}{}{}{}{}\ottprodnewline
\ottprodline{|}{\langle  \ottnt{labels}  \rangle}{}{}{}{}\ottprodnewline
\ottprodline{|}{\langle  \ottnt{labels}  \ottsym{,}  \varepsilon  \rangle} {\textsf{S}}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{atomic\_eff}} {\textsf{S}}{}{}{}}

\newcommand{\ottlabels}{
\ottrulehead{\ottnt{labels}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottnt{label}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{label_{{\mathrm{1}}}}  \ottsym{,}  \ldots  \ottsym{,}  \ottnt{label_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{labels_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{labels_{{\mathrm{2}}}}}{}{}{}{}}

\newcommand{\ottseq}{
\ottrulehead{\varepsilon}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\rho}{}{}{}{}\ottprodnewline
\ottprodline{|}{ [] }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{[}  \ottnt{label}  \ottsym{]}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\varepsilon_{{\mathrm{1}}}  \ottsym{;}  \varepsilon_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{atomic\_eff}} {\textsf{S}}{}{}{}}

\newcommand{\ottSet}{
\ottrulehead{{s}  ,\ \varepsilon}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\rho}{}{}{}{}\ottprodnewline
\ottprodline{|}{\{  \}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\{  \ottnt{labels}  \}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {s}_{{\mathrm{1}}}  \,\underline{ \cup }\,  {s}_{{\mathrm{2}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {s}_{{\mathrm{1}}}  \,\underline{ \sqcup }\,  {s}_{{\mathrm{2}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {s}_{{\mathrm{1}}}  \,\underline{ \cup }\, \cdots \,\underline{ \cup }\,  {s}_{{\mathrm{2}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {s}_{{\mathrm{1}}}  \,\underline{ \sqcup }\, \cdots \,\underline{ \sqcup }\,  {s}_{{\mathrm{2}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {s}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{atomic\_eff}} {\textsf{S}}{}{}{}}

\newcommand{\ottsimrel}{
\ottrulehead{\otterr{Undefined}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\sim}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_{\eanameSet} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_{\eanameMSet} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_\mathrm{ESet} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_\mathrm{EMSet} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_{\eanameSimpleRow} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_{\eanameEraseSimpleRow} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_{\eanameScopedRow} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_{\eanameEraseScopedRow} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_\mathrm{ESimpR} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sim_\mathrm{EScpR} }{}{}{}{}}

\newcommand{\ottpsi}{
\ottrulehead{\psi  ,\ \phi}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \varepsilon_{{\mathrm{1}}}  \olessthan  \varepsilon_{{\mathrm{2}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{joined\_eff_{{\mathrm{1}}}}   \otterr{Undefined}   \ottnt{joined\_eff_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{joined\_eff_{{\mathrm{1}}}}   \nsim   \ottnt{joined\_eff_{{\mathrm{2}}}} }{}{}{}{}}

\newcommand{\ottodotop}{
\ottrulehead{\otterr{Undefined}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\odot}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \odot_\mathrm{SimpR} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \odot_\mathrm{ScpR} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \odot_\mathrm{ESimpR} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \odot_\mathrm{EScpR} }{}{}{}{}}

\newcommand{\ottjoinedXXeff}{
\ottrulehead{\ottnt{joined\_eff}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\varepsilon}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{joined\_eff_{{\mathrm{1}}}}  \mathop{ \otterr{Undefined} }  \ottnt{joined\_eff_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{joined\_eff_{{\mathrm{1}}}}  \mathop{ \otterr{Undefined}_{{\mathrm{1}}} } \cdots \mathop{ \otterr{Undefined}_{{\mathrm{2}}} }  \ottnt{joined\_eff_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{joined\_eff}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottatomicXXeff}{
\ottrulehead{\ottnt{atomic\_eff}  ,\ a  ,\ b}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottsym{-}}{}{}{}{}}

\newcommand{\ottA}{
\ottrulehead{\ottnt{A}  ,\ \ottnt{B}  ,\ \ottnt{C}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\tau}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{A}   \ottnt{Arrow}   \ottnt{B} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{Forall}   \ottnt{A}   \ottnt{UpEff} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \psi   \Rightarrow   \ottnt{A}   \ottnt{UpEff} }{}{}{}{}}

\newcommand{\ottU}{
\ottrulehead{S  ,\ T}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\varepsilon}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{label}}{}{}{}{}\ottprodnewline
\ottprodline{|}{S \, \ottnt{SubstType}}{}{}{}{}}

\newcommand{\ottK}{
\ottrulehead{\ottnt{K}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \mathbf{Typ} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathbf{Lab} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathbf{Eff} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Kinds}  \rightarrow  \ottnt{K}}{}{}{}{}}

\newcommand{\ottUs}{
\ottrulehead{\ottnt{Us}  ,\ \ottnt{Vs}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ {} }{}{}{}{}\ottprodnewline
\ottprodline{|}{S}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \bm{ { S } } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \bm{ { S } } ^ {  \mathit{I}  } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Us}  \ottsym{,}  \ottnt{Vs}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Us}  \ottsym{,}  \ldots  \ottsym{,}  \ottnt{Vs}}{}{}{}{}}

\newcommand{\ottLParams}{
\ottrulehead{\mathcal{P}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \bullet }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{Us}  \blacktriangleright  \mathcal{P} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{Us}  \blacktriangleright \cdots \blacktriangleright  \ottnt{Vs}  \blacktriangleright  \mathcal{P} }{}{}{}{}}

\newcommand{\ottUKinds}{
\ottrulehead{\ottnt{UKinds}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{S  \ottsym{:}  \ottnt{K}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \bm{ { S } }^{ \mathit{I} } : \bm{ \ottnt{K} }^{ \mathit{I} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \bm{ { S } } : \bm{ \ottnt{K} } }{}{}{}{}}

\newcommand{\ottXs}{
\ottrulehead{\ottnt{Xs}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ {} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{x}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \bm{  \mathit{x}  }^{ \mathit{I} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \bm{  \mathit{x}  } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Xs_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{Xs_{{\mathrm{2}}}}}{}{}{}{}}

\newcommand{\ottAlphas}{
\ottrulehead{\ottnt{Alphas}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ {} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\alpha}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \bm{ { \alpha } } ^ {  \mathit{I}  } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \bm{ { \alpha } } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\alpha  \ottsym{:}  \ottnt{K}}{}{}{}{}}

\newcommand{\ottAlphaSet}{
\ottrulehead{\ottnt{AlphaSet}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\{  \ottnt{Alphas}  \}}{}{}{}{}}

\newcommand{\ottXSet}{
\ottrulehead{\ottnt{XSet}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\{  \ottnt{Xs}  \}}{}{}{}{}}

\newcommand{\ottVars}{
\ottrulehead{\ottnt{Vars}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\{  \ottnt{VarSeq}  \}}{}{}{}{}}

\newcommand{\ottVarSeq}{
\ottrulehead{\ottnt{VarSeq}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{x}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\alpha}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{VarSeq_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{VarSeq_{{\mathrm{2}}}}}{}{}{}{}}

\newcommand{\ottForall}{
\ottrulehead{\ottnt{Forall}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \forall   \ottnt{Alphas}   \ottsym{.} }{}{}{}{}}

\newcommand{\ottKinds}{
\ottrulehead{\ottnt{Kinds}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottnt{K}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\bm{ { \ottnt{K} } } }^{ \mathit{I} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\bm{ { \ottnt{K} } } } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Pi {\bm{ { \ottnt{K} } } }^{ \mathit{I} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Pi  \ottnt{DownIndex}   \ottnt{K_{\ottmv{i}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Pi {\bm{ { \ottnt{K} } } } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{K_{{\mathrm{1}}}}  \times  \ottnt{K_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{K_{{\mathrm{1}}}}  \times  \cdots  \times  \ottnt{K_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{Kinds}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottSubstType}{
\ottrulehead{\ottnt{SubstType}}{::=}{}}

\newcommand{\ottSubst}{
\ottrulehead{\ottnt{Subst}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \! [  \ottnt{v}  /  \mathit{x}  ] }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \! [ {\bm{ { \ottnt{v} } } }^{ \mathit{I} } / {\bm{ { \mathit{x}  } } }^{ \mathit{I} } ] }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \! [ {\bm{ { \ottnt{v} } } } / {\bm{ { \mathit{x}  } } } ] }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{SubstType}}{}{}{}{}}

\newcommand{\ottsig}{
\ottrulehead{\sigma}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottsym{\{}  \ottnt{ops}  \ottsym{\}}  \ottnt{UpIndex}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{}  \ottnt{ops}  \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \{\} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \sigma_{{\mathrm{1}}}   \uplus   \sigma_{{\mathrm{2}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\sigma \, \ottnt{SubstType}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \sigma  \ottsym{)}}{}{}{}{}}

\newcommand{\ottops}{
\ottrulehead{\ottnt{ops}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathsf{op}  \ottsym{:}  \ottnt{opsig}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{ops_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{ops_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{ops_{{\mathrm{1}}}}  \ottsym{,}  \ldots  \ottsym{,}  \ottnt{ops_{{\mathrm{2}}}}}{}{}{}{}}

\newcommand{\ottopsig}{
\ottrulehead{\ottnt{opsig}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \ottnt{A}   \Rightarrow   \ottnt{B} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{Forall}   \ottnt{A}   \Rightarrow   \ottnt{B} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\Xi  \ottsym{(}  \mathit{l}  \ottsym{)}  \ottsym{(}  \ottnt{Us}  \ottsym{)}  \ottsym{(}  \mathsf{op}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottG}{
\ottrulehead{\Gamma}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\emptyset}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{x}  \ottsym{:}  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma \, \ottnt{SubstType}}{}{}{}{}}

\newcommand{\ottD}{
\ottrulehead{\Delta}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\emptyset}{}{}{}{}\ottprodnewline
\ottprodline{|}{\alpha  \ottsym{:}  \ottnt{K}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Delta \, \ottnt{SubstType}}{}{}{}{}}

\newcommand{\ottP}{
\ottrulehead{P}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\emptyset}{}{}{}{}\ottprodnewline
\ottprodline{|}{\psi}{}{}{}{}\ottprodnewline
\ottprodline{|}{P \, \ottnt{SubstType}}{}{}{}{}}

\newcommand{\ottS}{
\ottrulehead{\Xi}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\emptyset}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathit{l}  ::  \ottnt{LDecl} }{}{}{}{}}

\newcommand{\ottLDecl}{
\ottrulehead{\ottnt{LDecl}}{::=}{}}

\newcommand{\ottSig}{
\ottrulehead{\Sigma}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\Sbase}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Slabel}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Sigma_{{\mathrm{1}}}   \uplus   \Sigma_{{\mathrm{2}}} }{}{}{}{}}

\newcommand{\ottARE}{
\ottrulehead{\ottnt{ARE}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\Delta  \vdash  \psi}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Delta  \not\vdash  \psi}{}{}{}{}}

\newcommand{\ottE}{
\ottrulehead{\ottnt{E}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\Box}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathbf{let} \, \mathit{x}  \ottsym{=}  \ottnt{E} \, \mathbf{in} \, \ottnt{e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Handle} \, \ottnt{E} \, \mathbf{with} \, \ottnt{h}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Handle} \, \ottnt{E} \, \mathbf{with} \, \ottnt{varh}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathbf{if} \, \ottnt{E} \, \mathbf{then} \, \ottnt{e_{{\mathrm{2}}}} \, \mathbf{else} \, \ottnt{e_{{\mathrm{3}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{E}  ] _{ \ottnt{L} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\langle  c  \rangle  \ottnt{E}}{}{}{}{}}

\newcommand{\ottConstructor}{
\ottrulehead{\ottnt{Constructor}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathbf{let} \, \ottnt{PlaceHolder} \, \mathbf{in}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Handle} \, \ottnt{PlaceHolder} \, \mathbf{with}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottkw{fun} \, \ottsym{(}  \ottnt{PlaceHolder_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{PlaceHolder_{{\mathrm{2}}}}  \ottsym{,}  \ottnt{PlaceHolder_{{\mathrm{3}}}}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ [\,  \ottnt{PlaceHolder} \, ] _{ \ottnt{label} } }{}{}{}{}}

\newcommand{\ottPlaceHolder}{
\ottrulehead{\ottnt{PlaceHolder}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \!\textnormal{--}\! }{}{}{}{}}

\newcommand{\ottHandle}{
\ottrulehead{\ottnt{Handle}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \mathbf{handle}_{ \ottnt{label} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathbf{handle} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\mathbf{handle}\mathrm{-}\mathbf{var} }_{ \ottnt{label} } }{}{}{}{}}

\newcommand{\ottOP}{
\ottrulehead{\ottnt{OP}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \mathsf{op} _{ \ottnt{label} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{op} }{}{}{}{}}

\newcommand{\ottArrow}{
\ottrulehead{\ottnt{Arrow}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \rightarrow_{ \varepsilon } }{}{}{}{}}

\newcommand{\ottUpEff}{
\ottrulehead{\ottnt{UpEff}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ ^{ \varepsilon } }{}{}{}{}}

\newcommand{\ottUpIndex}{
\ottrulehead{\ottnt{UpIndex}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ ^{ \ottmv{i}  \in  \mathit{I} } }{}{}{}{}}

\newcommand{\ottDownIndex}{
\ottrulehead{\ottnt{DownIndex}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ _{ \ottmv{i}  \in  \mathit{I} } }{}{}{}{}}

\newcommand{\ottDom}{
\ottrulehead{\ottnt{Dom}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\emptyset}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{AlphaSet}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{Vars}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathrm{dom}   \ottsym{(}   \Gamma   \ottsym{)} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{Dom_{{\mathrm{1}}}}   \cap   \ottnt{Dom_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{Dom_{{\mathrm{1}}}}   \cup   \ottnt{Dom_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{Dom_{{\mathrm{1}}}}   \setminus   \ottnt{Dom_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{Dom}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottFreeVar}{
\ottrulehead{\ottnt{FreeVar}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\emptyset}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{XSet}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathrm{FV}   \ottsym{(}   \ottnt{e}   \ottsym{)} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{FreeVar_{{\mathrm{1}}}}   \cap   \ottnt{FreeVar_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{FreeVar_{{\mathrm{1}}}}   \cup   \ottnt{FreeVar_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{FreeVar_{{\mathrm{1}}}}   \setminus   \ottnt{FreeVar_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{FreeVar}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottFreeTVar}{
\ottrulehead{\ottnt{FreeTVar}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\emptyset}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{AlphaSet}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathrm{FTV}   \ottsym{(}   \ottnt{e}   \ottsym{)} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathrm{FTV}   \ottsym{(}   \ottnt{Us}   \ottsym{)} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{FreeTVar_{{\mathrm{1}}}}   \cap   \ottnt{FreeTVar_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{FreeTVar_{{\mathrm{1}}}}   \cup   \ottnt{FreeTVar_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{FreeTVar_{{\mathrm{1}}}}   \setminus   \ottnt{FreeTVar_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{FreeTVar}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottgrammar}{\ottgrammartabular{
\otte\ottinterrule
\ottv\ottinterrule
\ottco\ottinterrule
\ottconst\ottinterrule
\ottnum\ottinterrule
\otth\ottinterrule
\ottvarh\ottinterrule
\otthClause\ottinterrule
\ottupluses\ottinterrule
\ottlabel\ottinterrule
\ottepsilon\ottinterrule
\ottrow\ottinterrule
\ottlabels\ottinterrule
\ottseq\ottinterrule
\ottSet\ottinterrule
\ottsimrel\ottinterrule
\ottpsi\ottinterrule
\ottodotop\ottinterrule
\ottjoinedXXeff\ottinterrule
\ottatomicXXeff\ottinterrule
\ottA\ottinterrule
\ottU\ottinterrule
\ottK\ottinterrule
\ottUs\ottinterrule
\ottLParams\ottinterrule
\ottUKinds\ottinterrule
\ottXs\ottinterrule
\ottAlphas\ottinterrule
\ottAlphaSet\ottinterrule
\ottXSet\ottinterrule
\ottVars\ottinterrule
\ottVarSeq\ottinterrule
\ottForall\ottinterrule
\ottKinds\ottinterrule
\ottSubstType\ottinterrule
\ottSubst\ottinterrule
\ottsig\ottinterrule
\ottops\ottinterrule
\ottopsig\ottinterrule
\ottG\ottinterrule
\ottD\ottinterrule
\ottP\ottinterrule
\ottS\ottinterrule
\ottLDecl\ottinterrule
\ottSig\ottinterrule
\ottARE\ottinterrule
\ottE\ottinterrule
\ottConstructor\ottinterrule
\ottPlaceHolder\ottinterrule
\ottHandle\ottinterrule
\ottOP\ottinterrule
\ottArrow\ottinterrule
\ottUpEff\ottinterrule
\ottUpIndex\ottinterrule
\ottDownIndex\ottinterrule
\ottDom\ottinterrule
\ottFreeVar\ottinterrule
\ottFreeTVar\ottafterlastrule
}}

% defnss
% defns Jtype
%% defn context_wellformedness
\newcommand{\ottdruleCXXEmpty}[1]{\ottdrule[#1]{%
}{
\vdash  \emptyset}{%
{\ottdrulename{C\_Empty}}{}%
}}


\newcommand{\ottdruleCXXVar}[1]{\ottdrule[#1]{%
\ottpremise{  \mathit{x}   \notin    \mathrm{dom}   \ottsym{(}   \Gamma   \ottsym{)}    \quad \quad  \Gamma  \vdash  \ottnt{A}  \ottsym{:}   \mathbf{Typ}  }%
}{
\vdash  \Gamma  \ottsym{,}  \mathit{x}  \ottsym{:}  \ottnt{A}}{%
{\ottdrulename{C\_Var}}{}%
}}


\newcommand{\ottdruleCXXTVar}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash  \Gamma  \quad \quad   \alpha   \notin    \mathrm{dom}   \ottsym{(}   \Gamma   \ottsym{)}   }%
}{
\vdash  \Gamma  \ottsym{,}  \alpha  \ottsym{:}  \ottnt{K}}{%
{\ottdrulename{C\_TVar}}{}%
}}


\newcommand{\ottdruleCXXPred}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \vdash  \psi}%
}{
\vdash  \Gamma  \ottsym{,}  \psi}{%
{\ottdrulename{C\_Pred}}{}%
}}

\newcommand{\ottdefncontextXXwellformedness}[1]{\begin{ottdefnblock}[#1]{$\vdash  \Gamma$}{\ottcom{well-formed context}}
\ottusedrule{\ottdruleCXXEmpty{}}
\ottusedrule{\ottdruleCXXVar{}}
\ottusedrule{\ottdruleCXXTVar{}}
\ottusedrule{\ottdruleCXXPred{}}
\end{ottdefnblock}}

%% defn wellformed_predicate
\newcommand{\ottdrulePXXPreOne}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \varepsilon_{{\mathrm{1}}}  \ottsym{:}   \mathbf{Eff}   \quad \quad  \Gamma  \vdash  \varepsilon_{{\mathrm{2}}}  \ottsym{:}   \mathbf{Eff}  }%
}{
\Gamma  \vdash   \varepsilon_{{\mathrm{1}}}  \olessthan  \varepsilon_{{\mathrm{2}}} }{%
{\ottdrulename{P\_Pre1}}{}%
}}


\newcommand{\ottdrulePXXPreTwo}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \varepsilon_{{\mathrm{1}}}  \ottsym{:}   \mathbf{Eff}   \quad \quad  \Gamma  \vdash  \varepsilon_{{\mathrm{2}}}  \ottsym{:}   \mathbf{Eff}   \quad \quad  \Gamma  \vdash  \varepsilon_{{\mathrm{3}}}  \ottsym{:}   \mathbf{Eff}  }%
}{
\Gamma  \vdash    \varepsilon_{{\mathrm{1}}}  \mathop{ \odot }  \varepsilon_{{\mathrm{2}}}    \sim   \varepsilon_{{\mathrm{3}}} }{%
{\ottdrulename{P\_Pre2}}{}%
}}

\newcommand{\ottdefnwellformedXXpredicate}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \psi$}{\ottcom{well-formed predicate}}
\ottusedrule{\ottdrulePXXPreOne{}}
\ottusedrule{\ottdrulePXXPreTwo{}}
\end{ottdefnblock}}

%% defn kinding
\newcommand{\ottdruleKXXVar}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash  \Gamma  \quad \quad   \alpha   \ottsym{:}   \ottnt{K}   \in   \Gamma  }%
}{
\Gamma  \vdash  \alpha  \ottsym{:}  \ottnt{K}}{%
{\ottdrulename{K\_Var}}{}%
}}


\newcommand{\ottdruleKXXLabel}[1]{\ottdrule[#1]{%
\ottpremise{  \mathit{l}  ::    \forall    {\bm{ \alpha } }^{ \mathit{I} } : {\bm{ \ottnt{K} } }^{ \mathit{I} }    \ottsym{.}    \sigma    \in   \Xi   \quad \quad  \Gamma  \vdash   \bm{ { S } }^{ \mathit{I} } : \bm{ \ottnt{K} }^{ \mathit{I} }  }%
}{
\Gamma  \vdash  \mathit{l} \,  \bm{ { S } } ^ {  \mathit{I}  }   \ottsym{:}   \mathbf{Lab} }{%
{\ottdrulename{K\_Label}}{}%
}}


\newcommand{\ottdruleKXXFun}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{A}  \ottsym{:}   \mathbf{Typ}   \quad \quad  \Gamma  \vdash  \varepsilon  \ottsym{:}   \mathbf{Eff}   \quad \quad  \Gamma  \vdash  \ottnt{B}  \ottsym{:}   \mathbf{Typ}  }%
}{
\Gamma  \vdash   \ottnt{A}    \rightarrow_{ \varepsilon }    \ottnt{B}   \ottsym{:}   \mathbf{Typ} }{%
{\ottdrulename{K\_Fun}}{}%
}}


\newcommand{\ottdruleKXXPoly}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \ottsym{,}  \alpha  \ottsym{:}  \ottnt{K}  \vdash  \ottnt{A}  \ottsym{:}   \mathbf{Typ}   \quad \quad  \Gamma  \ottsym{,}  \alpha  \ottsym{:}  \ottnt{K}  \vdash  \varepsilon  \ottsym{:}   \mathbf{Eff}  }%
}{
\Gamma  \vdash    \forall   \alpha  \ottsym{:}  \ottnt{K}   \ottsym{.}    \ottnt{A}    ^{ \varepsilon }    \ottsym{:}   \mathbf{Typ} }{%
{\ottdrulename{K\_Poly}}{}%
}}


\newcommand{\ottdruleKXXPred}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \ottsym{,}  \psi  \vdash  \ottnt{A}  \ottsym{:}   \mathbf{Typ}   \quad \quad  \Gamma  \ottsym{,}  \psi  \vdash  \varepsilon  \ottsym{:}   \mathbf{Eff}  }%
}{
\Gamma  \vdash   \psi   \Rightarrow   \ottnt{A}    ^{ \varepsilon }    \ottsym{:}   \mathbf{Typ} }{%
{\ottdrulename{K\_Pred}}{}%
}}


\newcommand{\ottdruleKXXCons}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash  \Gamma  \quad \quad   \mathcal{C}   \ottsym{:}    {\bm{ { \ottnt{K} } } }^{ \mathit{I} }   \rightarrow  \ottnt{K}   \in    \Slabel   \uplus   \Sbase    \quad \quad  \Gamma  \vdash   \bm{ { S } }^{ \mathit{I} } : \bm{ \ottnt{K} }^{ \mathit{I} }  }%
}{
\Gamma  \vdash  \mathcal{C} \,  \bm{ { S } } ^ {  \mathit{I}  }   \ottsym{:}  \ottnt{K}}{%
{\ottdrulename{K\_Cons}}{}%
}}

\newcommand{\ottdefnkinding}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \ottnt{UKinds}$}{}
\ottusedrule{\ottdruleKXXVar{}}
\ottusedrule{\ottdruleKXXLabel{}}
\ottusedrule{\ottdruleKXXFun{}}
\ottusedrule{\ottdruleKXXPoly{}}
\ottusedrule{\ottdruleKXXPred{}}
\ottusedrule{\ottdruleKXXCons{}}
\end{ottdefnblock}}

%% defn typing
\newcommand{\ottdruleTXXVar}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash  \Gamma  \quad \quad   \mathit{x}   \ottsym{:}   \ottnt{A}   \in   \Gamma  }%
}{
\Gamma  \vdash  \mathit{x}  \ottsym{:}  \ottnt{A}  \mid   \bbZero }{%
{\ottdrulename{T\_Var}}{}%
}}


\newcommand{\ottdruleTXXAbs}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \ottsym{,}  \mathit{g}  \ottsym{:}   \ottnt{A}    \rightarrow_{ \varepsilon }    \ottnt{B}   \ottsym{,}  \mathit{x}  \ottsym{:}  \ottnt{A}  \vdash  \ottnt{e}  \ottsym{:}  \ottnt{B}  \mid  \varepsilon}%
}{
\Gamma  \vdash  \ottkw{fun} \, \ottsym{(}  \mathit{g}  \ottsym{,}  \mathit{x}  \ottsym{,}  \ottnt{e}  \ottsym{)}  \ottsym{:}   \ottnt{A}    \rightarrow_{ \varepsilon }    \ottnt{B}   \mid   \bbZero }{%
{\ottdrulename{T\_Abs}}{}%
}}


\newcommand{\ottdruleTXXApp}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{v_{{\mathrm{1}}}}  \ottsym{:}   \ottnt{A}    \rightarrow_{ \varepsilon }    \ottnt{B}   \mid   \bbZero   \quad \quad  \Gamma  \vdash  \ottnt{v_{{\mathrm{2}}}}  \ottsym{:}  \ottnt{A}  \mid   \bbZero  }%
}{
\Gamma  \vdash  \ottnt{v_{{\mathrm{1}}}} \, \ottnt{v_{{\mathrm{2}}}}  \ottsym{:}  \ottnt{B}  \mid  \varepsilon}{%
{\ottdrulename{T\_App}}{}%
}}


\newcommand{\ottdruleTXXTAbs}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \ottsym{,}  \alpha  \ottsym{:}  \ottnt{K}  \vdash  \ottnt{e}  \ottsym{:}  \ottnt{A}  \mid  \varepsilon}%
}{
\Gamma  \vdash  \Lambda  \alpha  \ottsym{:}  \ottnt{K}  \ottsym{.}  \ottnt{e}  \ottsym{:}    \forall   \alpha  \ottsym{:}  \ottnt{K}   \ottsym{.}    \ottnt{A}    ^{ \varepsilon }    \mid   \bbZero }{%
{\ottdrulename{T\_TAbs}}{}%
}}


\newcommand{\ottdruleTXXTApp}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{v}  \ottsym{:}    \forall   \alpha  \ottsym{:}  \ottnt{K}   \ottsym{.}    \ottnt{A}    ^{ \varepsilon }    \mid   \bbZero   \quad \quad  \Gamma  \vdash  S  \ottsym{:}  \ottnt{K} }%
}{
\Gamma  \vdash  \ottnt{v} \, S  \ottsym{:}  \ottnt{A} \,  \! [  S  /  \alpha   ]   \mid  \varepsilon \,  \! [  S  /  \alpha   ] }{%
{\ottdrulename{T\_TApp}}{}%
}}


\newcommand{\ottdruleTXXPAbs}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \ottsym{,}  \psi  \vdash  \ottnt{e}  \ottsym{:}  \ottnt{A}  \mid  \varepsilon}%
}{
\Gamma  \vdash  \psi  \Rightarrow  \ottnt{e}  \ottsym{:}   \psi   \Rightarrow   \ottnt{A}    ^{ \varepsilon }    \mid   \bbZero }{%
{\ottdrulename{T\_PAbs}}{}%
}}


\newcommand{\ottdruleTXXPApp}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{v}  \ottsym{:}   \psi   \Rightarrow   \ottnt{A}    ^{ \varepsilon }    \mid   \bbZero   \quad \quad   \Delta   \ottsym{(}   \Gamma   \ottsym{)}   \vdash  \psi }%
}{
\Gamma  \vdash  \ottnt{v} \, \psi  \ottsym{:}  \ottnt{A}  \mid  \varepsilon}{%
{\ottdrulename{T\_PApp}}{}%
}}


\newcommand{\ottdruleTXXLet}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{e_{{\mathrm{1}}}}  \ottsym{:}  \ottnt{A}  \mid  \varepsilon  \quad \quad  \Gamma  \ottsym{,}  \mathit{x}  \ottsym{:}  \ottnt{A}  \vdash  \ottnt{e_{{\mathrm{2}}}}  \ottsym{:}  \ottnt{B}  \mid  \varepsilon }%
}{
\Gamma  \vdash  \mathbf{let} \, \mathit{x}  \ottsym{=}  \ottnt{e_{{\mathrm{1}}}} \, \mathbf{in} \, \ottnt{e_{{\mathrm{2}}}}  \ottsym{:}  \ottnt{B}  \mid  \varepsilon}{%
{\ottdrulename{T\_Let}}{}%
}}


\newcommand{\ottdruleTXXSub}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{e}  \ottsym{:}  \ottnt{A}  \mid  \varepsilon  \quad \quad  \Gamma  \vdash  \ottnt{A}  <:  \ottnt{A'}  \quad \quad   \Delta   \ottsym{(}   \Gamma   \ottsym{)}   \vdash   \varepsilon  \olessthan  \varepsilon'  }%
}{
\Gamma  \vdash  \ottnt{e}  \ottsym{:}  \ottnt{A'}  \mid  \varepsilon'}{%
{\ottdrulename{T\_Sub}}{}%
}}


\newcommand{\ottdruleTXXOp}[1]{\ottdrule[#1]{%
\ottpremise{  \mathit{l}  ::    \forall    {\bm{ \alpha } }^{ \mathit{I} } : {\bm{ \ottnt{K} } }^{ \mathit{I} }    \ottsym{.}    \sigma    \in   \Xi   \quad \quad   \mathsf{op}  \ottsym{:}    \forall    {\bm{ \beta } }^{ \mathit{J} } : {\bm{ \ottnt{K'} } }^{ \mathit{J} }    \ottsym{.}    \ottnt{A}   \Rightarrow   \ottnt{B}    \in   \sigma  }%
\ottpremise{ \Gamma  \vdash   \bm{ { S } }^{ \mathit{I} } : \bm{ \ottnt{K} }^{ \mathit{I} }   \quad \quad  \Gamma  \vdash   \bm{ { T } }^{ \mathit{J} } : \bm{ \ottnt{K'} }^{ \mathit{J} }  }%
}{
\Gamma  \vdash   \mathsf{op} _{ \mathit{l} \,  \bm{ { S } } ^ {  \mathit{I}  }  }  \,  \bm{ { T } } ^ {  \mathit{J}  }   \ottsym{:}   \ottsym{(}  \ottnt{A} \,  \! [ {\bm{ { S } } }^{ \mathit{I} } / {\bm{ \alpha } }^{ \mathit{I} } ]  \,  \! [ {\bm{ { T } } }^{ \mathit{J} } / {\bm{ \beta } }^{ \mathit{J} } ]   \ottsym{)}    \rightarrow_{  \lift{ \ottsym{(}  \mathit{l} \,  \bm{ { S } } ^ {  \mathit{I}  }   \ottsym{)} }  }    \ottsym{(}  \ottnt{B} \,  \! [ {\bm{ { S } } }^{ \mathit{I} } / {\bm{ \alpha } }^{ \mathit{I} } ]  \,  \! [ {\bm{ { T } } }^{ \mathit{J} } / {\bm{ \beta } }^{ \mathit{J} } ]   \ottsym{)}   \mid   \bbZero }{%
{\ottdrulename{T\_Op}}{}%
}}


\newcommand{\ottdruleTXXHandling}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{e}  \ottsym{:}  \ottnt{A}  \mid  \varepsilon  \quad \quad  \Gamma  \ottsym{,}  \mathit{x}  \ottsym{:}  \ottnt{A}  \vdash  \ottnt{e_{\ottmv{r}}}  \ottsym{:}  \ottnt{C}  \mid  \varepsilon'  \quad \quad   \Delta   \ottsym{(}   \Gamma   \ottsym{)}   \vdash     \lift{ \ottsym{(}  \mathit{l} \,  \bm{ { S } } ^ {  \mathit{N}  }   \ottsym{)} }   \mathop{ \odot }  \varepsilon'    \sim   \varepsilon  }%
\ottpremise{ \Gamma  \vdash _{ \mathit{l}  \, \bm{ { S } }^{ \mathit{N} } } \{  \mathsf{op_{\ottmv{i}}} \, \bm{ \beta_{\ottmv{i}} }^{ \mathit{J_{\ottmv{i}}} } : \bm{ \ottnt{K_{\ottmv{i}}} }^{ \mathit{J_{\ottmv{i}}} } \,  \mathit{p_{\ottmv{i}}}  \,  \mathit{k_{\ottmv{i}}}  \mapsto  \ottnt{e_{\ottmv{i}}}  \} ^{ \ottmv{i}  \in  \mathit{I} } :  \ottnt{C}  \mid  \varepsilon' }%
}{
\Gamma  \vdash   \mathbf{handle}_{ \mathit{l} \,  \bm{ { S } } ^ {  \mathit{N}  }  }  \, \ottnt{e} \, \mathbf{with} \,  \ottsym{\{} \, \mathbf{return} \, \mathit{x}  \mapsto  \ottnt{e_{\ottmv{r}}}  \ottsym{\}}   \uplus   \ottsym{\{}  \mathsf{op_{\ottmv{i}}} \,  {\bm{ \beta_{\ottmv{i}} } }^{ \mathit{J_{\ottmv{i}}} } : {\bm{ \ottnt{K_{\ottmv{i}}} } }^{ \mathit{J_{\ottmv{i}}} }  \, \mathit{p_{\ottmv{i}}} \, \mathit{k_{\ottmv{i}}}  \mapsto  \ottnt{e_{\ottmv{i}}}  \ottsym{\}}   ^{ \ottmv{i}  \in  \mathit{I} }    \ottsym{:}  \ottnt{C}  \mid  \varepsilon'}{%
{\ottdrulename{T\_Handling}}{}%
}}

\newcommand{\ottdefntyping}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \ottnt{e}  \ottsym{:}  \ottnt{A}  \mid  \varepsilon$}{\ottcom{Typing}}
\ottusedrule{\ottdruleTXXVar{}}
\ottusedrule{\ottdruleTXXAbs{}}
\ottusedrule{\ottdruleTXXApp{}}
\ottusedrule{\ottdruleTXXTAbs{}}
\ottusedrule{\ottdruleTXXTApp{}}
\ottusedrule{\ottdruleTXXPAbs{}}
\ottusedrule{\ottdruleTXXPApp{}}
\ottusedrule{\ottdruleTXXLet{}}
\ottusedrule{\ottdruleTXXSub{}}
\ottusedrule{\ottdruleTXXOp{}}
\ottusedrule{\ottdruleTXXHandling{}}
\end{ottdefnblock}}

%% defn opClauses
\newcommand{\ottdruleHXXAux}[1]{\ottdrule[#1]{%
\ottpremise{ \mathit{l}  ::    \forall    {\bm{ \alpha } }^{ \mathit{N} } : {\bm{ \ottnt{K} } }^{ \mathit{N} }    \ottsym{.}    \ottsym{\{}  \mathsf{op_{\ottmv{i}}}  \ottsym{:}    \forall    {\bm{ \beta_{\ottmv{i}} } }^{ \mathit{J_{\ottmv{i}}} } : {\bm{ \ottnt{K_{\ottmv{i}}} } }^{ \mathit{J_{\ottmv{i}}} }    \ottsym{.}    \ottnt{A_{\ottmv{i}}}   \Rightarrow   \ottnt{B_{\ottmv{i}}}   \ottsym{\}}   ^{ \ottmv{i}  \in  \mathit{I} }     \in   \Xi }%
\ottpremise{\ottcomp{\Gamma  \ottsym{,}   {\bm{ \beta_{\ottmv{i}} } }^{ \mathit{J_{\ottmv{i}}} } : {\bm{ \ottnt{K_{\ottmv{i}}} } }^{ \mathit{J_{\ottmv{i}}} }   \ottsym{,}  \mathit{p_{\ottmv{i}}}  \ottsym{:}  \ottnt{A_{\ottmv{i}}} \,  \! [ {\bm{ { S } } }^{ \mathit{N} } / {\bm{ \alpha } }^{ \mathit{N} } ]   \ottsym{,}  \mathit{k_{\ottmv{i}}}  \ottsym{:}   \ottnt{B_{\ottmv{i}}} \,  \! [ {\bm{ { S } } }^{ \mathit{N} } / {\bm{ \alpha } }^{ \mathit{N} } ]     \rightarrow_{ \varepsilon }    \ottnt{C}   \vdash  \ottnt{e_{\ottmv{i}}}  \ottsym{:}  \ottnt{C}  \mid  \varepsilon}{\ottmv{i}}}%
}{
 \Gamma  \vdash _{ \mathit{l}  \, \bm{ { S } }^{ \mathit{N} } } \{  \mathsf{op_{\ottmv{i}}} \, \bm{ \beta_{\ottmv{i}} }^{ \mathit{J_{\ottmv{i}}} } : \bm{ \ottnt{K_{\ottmv{i}}} }^{ \mathit{J_{\ottmv{i}}} } \,  \mathit{p_{\ottmv{i}}}  \,  \mathit{k_{\ottmv{i}}}  \mapsto  \ottnt{e_{\ottmv{i}}}  \} ^{ \ottmv{i}  \in  \mathit{I} } :  \ottnt{C}  \mid  \varepsilon }{%
{\ottdrulename{H\_Aux}}{}%
}}

\newcommand{\ottdefnopClauses}[1]{\begin{ottdefnblock}[#1]{$ \Gamma  \vdash _{ \mathit{l}  \, \bm{ { S } }^{ \mathit{N} } } \{  \mathsf{op_{\ottmv{i}}} \, \bm{ \beta_{\ottmv{i}} }^{ \mathit{J_{\ottmv{i}}} } : \bm{ \ottnt{K_{\ottmv{i}}} }^{ \mathit{J_{\ottmv{i}}} } \,  \mathit{p_{\ottmv{i}}}  \,  \mathit{k_{\ottmv{i}}}  \mapsto  \ottnt{e_{\ottmv{i}}}  \} ^{ \ottmv{i}  \in  \mathit{I} } :  \ottnt{C}  \mid  \varepsilon $}{}
\ottusedrule{\ottdruleHXXAux{}}
\end{ottdefnblock}}

%% defn handler

\newcommand{\ottdefnhandler}[1]{\begin{ottdefnblock}[#1]{$ \Gamma  \vdash _{ \ottnt{L} }  \ottnt{h}  :  \ottnt{A}   \Rightarrow  ^ { \varepsilon }  \ottnt{B} $}{}
\end{ottdefnblock}}

%% defn handler_sig

\newcommand{\ottdefnhandlerXXsig}[1]{\begin{ottdefnblock}[#1]{$ \Gamma  \vdash _{ \sigma }  \ottnt{h}  :  \ottnt{A}   \Rightarrow  ^ { \varepsilon }  \ottnt{B} $}{}
\end{ottdefnblock}}

%% defn handler_sig_shallow

\newcommand{\ottdefnhandlerXXsigXXshallow}[1]{\begin{ottdefnblock}[#1]{$ \Gamma  \vdash _{ \sigma }  \ottnt{h}  :  \ottnt{A}  ^ { \varepsilon' }  \Rightarrow  ^ { \varepsilon }  \ottnt{B} $}{}
\end{ottdefnblock}}

%% defn subtyping
\newcommand{\ottdruleSTXXRefl}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \vdash  \ottnt{A}  \ottsym{:}   \mathbf{Typ} }%
}{
\Gamma  \vdash  \ottnt{A}  <:  \ottnt{A}}{%
{\ottdrulename{ST\_Refl}}{}%
}}


\newcommand{\ottdruleSTXXFun}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{A_{{\mathrm{2}}}}  <:  \ottnt{A_{{\mathrm{1}}}}  \quad \quad  \Gamma  \vdash  \ottnt{B_{{\mathrm{1}}}}  \mid  \varepsilon_{{\mathrm{1}}}  <:  \ottnt{B_{{\mathrm{2}}}}  \mid  \varepsilon_{{\mathrm{2}}} }%
}{
\Gamma  \vdash   \ottnt{A_{{\mathrm{1}}}}    \rightarrow_{ \varepsilon_{{\mathrm{1}}} }    \ottnt{B_{{\mathrm{1}}}}   <:   \ottnt{A_{{\mathrm{2}}}}    \rightarrow_{ \varepsilon_{{\mathrm{2}}} }    \ottnt{B_{{\mathrm{2}}}} }{%
{\ottdrulename{ST\_Fun}}{}%
}}


\newcommand{\ottdruleSTXXPoly}[1]{\ottdrule[#1]{%
\ottpremise{\Gamma  \ottsym{,}  \alpha  \ottsym{:}  \ottnt{K}  \vdash  \ottnt{A_{{\mathrm{1}}}}  \mid  \varepsilon_{{\mathrm{1}}}  <:  \ottnt{A_{{\mathrm{2}}}}  \mid  \varepsilon_{{\mathrm{2}}}}%
}{
\Gamma  \vdash    \forall   \alpha  \ottsym{:}  \ottnt{K}   \ottsym{.}    \ottnt{A_{{\mathrm{1}}}}    ^{ \varepsilon_{{\mathrm{1}}} }    <:    \forall   \alpha  \ottsym{:}  \ottnt{K}   \ottsym{.}    \ottnt{A_{{\mathrm{2}}}}    ^{ \varepsilon_{{\mathrm{2}}} }  }{%
{\ottdrulename{ST\_Poly}}{}%
}}


\newcommand{\ottdruleSTXXPred}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \ottsym{,}  \psi_{{\mathrm{2}}}  \vdash  \ottnt{A_{{\mathrm{1}}}}  <:  \ottnt{A_{{\mathrm{2}}}}  \quad \quad   \Delta   \ottsym{(}   \Gamma  \ottsym{,}  \psi_{{\mathrm{2}}}   \ottsym{)}   \vdash   \varepsilon_{{\mathrm{1}}}  \olessthan  \varepsilon_{{\mathrm{2}}}   \quad \quad   \Delta   \ottsym{(}   \Gamma  \ottsym{,}  \psi_{{\mathrm{2}}}   \ottsym{)}   \vdash  \psi_{{\mathrm{1}}} }%
}{
\Gamma  \vdash   \psi_{{\mathrm{1}}}   \Rightarrow   \ottnt{A_{{\mathrm{1}}}}    ^{ \varepsilon_{{\mathrm{1}}} }    <:   \psi_{{\mathrm{2}}}   \Rightarrow   \ottnt{A_{{\mathrm{2}}}}    ^{ \varepsilon_{{\mathrm{2}}} }  }{%
{\ottdrulename{ST\_Pred}}{}%
}}

\newcommand{\ottdefnsubtyping}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \ottnt{A}  <:  \ottnt{B}$}{\ottcom{subtyping}}
\ottusedrule{\ottdruleSTXXRefl{}}
\ottusedrule{\ottdruleSTXXFun{}}
\ottusedrule{\ottdruleSTXXPoly{}}
\ottusedrule{\ottdruleSTXXPred{}}
\end{ottdefnblock}}

%% defn subtyping_comp
\newcommand{\ottdruleSTXXComp}[1]{\ottdrule[#1]{%
\ottpremise{ \Gamma  \vdash  \ottnt{A}  <:  \ottnt{B}  \quad \quad   \Delta   \ottsym{(}   \Gamma   \ottsym{)}   \vdash   \varepsilon_{{\mathrm{1}}}  \olessthan  \varepsilon_{{\mathrm{2}}}  }%
}{
\Gamma  \vdash  \ottnt{A}  \mid  \varepsilon_{{\mathrm{1}}}  <:  \ottnt{B}  \mid  \varepsilon_{{\mathrm{2}}}}{%
{\ottdrulename{ST\_Comp}}{}%
}}

\newcommand{\ottdefnsubtypingXXcomp}[1]{\begin{ottdefnblock}[#1]{$\Gamma  \vdash  \ottnt{A}  \mid  \varepsilon  <:  \ottnt{B}  \mid  \varepsilon'$}{\ottcom{subtyping}}
\ottusedrule{\ottdruleSTXXComp{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsJtype}{
\ottdefncontextXXwellformedness{}\ottdefnwellformedXXpredicate{}\ottdefnkinding{}\ottdefntyping{}\ottdefnopClauses{}\ottdefnhandler{}\ottdefnhandlerXXsig{}\ottdefnhandlerXXsigXXshallow{}\ottdefnsubtyping{}\ottdefnsubtypingXXcomp{}}

% defns Jop
%% defn reduction

\newcommand{\ottdefnreduction}[1]{\begin{ottdefnblock}[#1]{$\ottnt{e_{{\mathrm{1}}}}  \longmapsto  \ottnt{e_{{\mathrm{2}}}}$}{\ottcom{reduction}}
\end{ottdefnblock}}

%% defn evaluation
\newcommand{\ottdruleEXXEval}[1]{\ottdrule[#1]{%
\ottpremise{\ottnt{e_{{\mathrm{1}}}}  \longmapsto  \ottnt{e_{{\mathrm{2}}}}}%
}{
\ottnt{E}  \ottsym{[}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{]}  \longrightarrow  \ottnt{E}  \ottsym{[}  \ottnt{e_{{\mathrm{2}}}}  \ottsym{]}}{%
{\ottdrulename{E\_Eval}}{}%
}}

\newcommand{\ottdefnevaluation}[1]{\begin{ottdefnblock}[#1]{$\ottnt{e_{{\mathrm{1}}}}  \longrightarrow  \ottnt{e_{{\mathrm{2}}}}$}{\ottcom{evaluation}}
\ottusedrule{\ottdruleEXXEval{}}
\end{ottdefnblock}}

%% defn wf_typelike_and_subst

\newcommand{\ottdefnwfXXtypelikeXXandXXsubst}[1]{\begin{ottdefnblock}[#1]{$ \alpha   \mapsto   S   \vdash   \ottnt{Us}  :  \ottnt{K} $}{}
\end{ottdefnblock}}


\newcommand{\ottdefnsJop}{
\ottdefnreduction{}\ottdefnevaluation{}\ottdefnwfXXtypelikeXXandXXsubst{}}

\newcommand{\ottdefnss}{
\ottdefnsJtype
\ottdefnsJop
}

\newcommand{\ottall}{\ottmetavars\\[0pt]
\ottgrammar\\[5.0mm]
\ottdefnss}



==> sections/discussion.tex <==
\section{Future Work}\label{sec:discussion}
% In this section, we discuss the further extensions of {\lang}: local effects and coercions.

% \subsection{Comparison of ARE instances}
% %
% \begin{table}[t]
%   \caption{Comparison of ARE Instances}
%   \label{tbl:comparison}
%   \begin{tabular}[t]{|c||c|c|c|}
%     \hline
%                 & Multiple effect variables & Type Erasability & Distinction of duplicate labels \\
%     \hline
%     Sets        & \cmark                    & \xmark           & \xmark                          \\
%     Simple Rows & \xmark                    & \cmark           & \xmark                          \\
%     Scoped Rows & \xmark                    & \cmark           & \cmark                          \\
%     Free Rows   & \cmark                    & \cmark           & \cmark                          \\
%     \hline
%   \end{tabular}
% \end{table}
% %
% We have provided four ARE instances: sets, simple rows, scoped rows, and free rows.
% %
% Their comparison is summarized in Table~\ref{tbl:comparison}.
% %
% We compare them from the following three perspectives:
% whether allowing multiple occurrences of effect variables,
% whether being extended to type-erasure semantics, and
% whether distinguishing multiple occurrences of labels from a single occurrence.

% As indicated by each effect signature of instances,
% sets and free rows allow multiple occurrences of effect variables,
% unlike simple rows and scoped rows.
% %
% This feature makes it possible to write a program like the one shown in Figure~\ref{fig:impl}.

% As discussed in Section~\ref{sec:erasure},
% instances other than sets can be adapted to the type-erasure semantics.
% %
% The feature that sets have no order makes adjusting to the type-erasure semantics difficult.

% As indicated by each equivalence relation of instances,
% sets and simple rows identify multiple occurrences of labels with a single occurrence.
% %
% This feature enables associating different handlers to different calls of the same operation,
% as introduced in Section~\ref{sec:overview}.

% Note that the practical application issues of free rows are unknown in contrast to the other three instances.
% %
% Thus, we cannot yet discuss the practical aspects of free rows comparing existing works of other instances~\ref{pretnar_inferring_2014, hillerstrom_liberating_2016, leijen_type_2017, biernacki_abstracting_2019, sekiyama_signature_2020}.

\TS{Other candidates to discuss: CPS translation, unification and type inference, sequential effects in abstract effect systems.}

\TS{This section needs to be revised.}

% Although effect representations by sets and simple row are similar, there are
% certain differences between them.

% To see them, let us compare sets in Example~\ref{exa:effset} and simple rows in
% Example~\ref{exa:eff_simple_row} first.
% %
% A main difference between them is that, while the set instance allows effect
% variables to occur anywhere in effects, the simple row instance restricts effect
% variables to appear only at the end of rows.
% %
% However, this difference is trivial \AI{straightforward? easy?} because we can define another
% instance of simple rows that allows non-restricted occurrences of effect
% variables, as in free rows presented in Section~\ref{sec:effseq}.
% %
% Note that simple rows only allows the exchange of different labels $\ottnt{L_{{\mathrm{1}}}}$ and
% $\ottnt{L_{{\mathrm{2}}}}$, while sets allow the exchange of any labels.
% %
% However, this does not differentiate the two instances because the prohibited
% exchange in simple rows, that is, the exchange of the same labels, is
% meaningless.

% Another difference is that it seems difficult to adapt the set instance to the
% type-erasure semantics unlike simple rows.
% %
% As seen in Section~\ref{sec:erasure}, rows are adapted to the type-erasure
% semantics by allowing only labels with different label names to be exchanged.
% %
% Because the set instance compares entire labels including typelike parameters,
% we cannot take this approach to adapt the set instance to the type-erasure
% semantics.

\subsection{Qualified Simple Rows}\label{subsec:q_simple_rows}

The original effect system with simple rows \citep{hillerstrom_liberating_2016}
differs from our effect system with simple rows (including both
Example~\ref{exa:eff_simple_row} and Example~\ref{exa:eff_simple_row_erasure})
at the two points: the original effect system \emph{syntactically} disallows
multiple labels to appear in a single row---while our simple rows identify
multiple occurrences and one occurrence of the same label
\emph{axiomatically}---and limits effect parameters passed to effect
abstractions for preserving that syntactic discipline.
%
To distinguish them, we call what the effect system of \citet{hillerstrom_liberating_2016} is based on
\emph{qualified simple rows}.

% An effect system with qualified simple rows realizes the features via its kind system shown below,
% in the setting where there are no parametric effects.
% %
% \begin{mathpar}
%   \inferrule{
%   \Gamma \vdash P : \mathbf{Presence} \\
%   \Gamma \vdash R : \mathbf{Row}_{\mathcal{L} \uplus \{l\} }
%   }{
%   \Gamma \vdash l : P ; R : \mathbf{Row}_{\mathcal{L}}
%   }

%   \inferrule{
%     \Gamma \vdash R : \mathbf{Row}_{\emptyset}
%   }{
%     \Gamma \vdash \{ R \} : \mathbf{Eff}
%   }
% \end{mathpar}
% %
% $P$ is the presence with types $\mathsf{Pre}(A)$ or the absence $\mathsf{Abs}$.
% $P = \mathsf{Pre}(A)$ represents that the row $l : P; R$ includes label $l$ typed as $A$.
% $P = \mathsf{Abs}$ represents that the row $l : P; R$ does not include label $l$.
% %
% The set $\mathcal{L}$ attached to $\mathbf{Row}$ denotes the labels uncovered by the row.
% %
% If $\mathcal{L}$ is the empty set, then the row can be the effect.
% %
% Therefore, all effects do not have multiple labels.
% %
% Furthermore, the instantiation of row variables is limited by this kind system.
% For example, consider the effect $\{l : \mathsf{Pre}(\ottnt{A}  \rightarrow  \ottnt{B}) ; \alpha\}$.
% We cannot substitute rows that have the field $l$ for the row variable $\alpha$,
% because the kind of $\alpha$ is $\mathbf{Row}_{\mathcal{L} \setminus \{l\}}$
% where $\mathcal{L}$ is the whole set of labels.

% To create an instance for qualified simple rows, we must extend {\lang}.
% Specifically, we need to add \emph{qualified types} to limit substitutions for effect variables.
% %
% Adding qualified types makes an ARE of qualified simple rows more complex
% because predicates in a context can be used.
% For example, an ARE for qualified simple rows at least satisfies the following: if $\{l\} \not\!\!\olessthan \alpha$ is in $\Delta$,
% then $\Delta \vdash \{l\} \odot \alpha \sim \{l, \alpha\}$ holds.
% %
% However, attaching qualified types to {\lang} seemingly does not affect safety conditions.
% % 
% Thus, the extension of {\lang} to cover qualified simple rows does not seem complex.

To address qualified simple rows, we have to extend {\lang}.
%
Specifically, we need to add \emph{qualified types}~\cite{jones_theory_1992, jones_theory_1994} to limit effects substituted
for effect variables.
%
Adding qualified types enables stating predicates on effects to be
met in typelike contexts.
%
Equipping {\lang} with qualified types seemingly does not affect safety conditions.
%
Thus, the extension of {\lang} with qualified types does not seem complex.
%
However, defining an effect algebra utilizing the assumed predicates is nontrivial.  For
example, an effect algebra for qualified simple rows should satisfy the following: if a
typelike context $ \Delta $ assumes that $\rho$ does not include $\mathit{l}$, then
$\Delta  \vdash    \langle  \mathit{l}  \rangle  \mathop{ \odot }  \rho    \sim   \langle  \mathit{l}  \mid  \rho  \rangle $ holds.
%
It is left open how such an effect algebra can be defined.

\subsection{Local Effects}\label{subsec:local_eff}
\TY{updated this part}

\emph{Local effects} are algebraic effects declared locally \citep{biernacki_abstracting_2019, vilhena_type_2023}.
%
For example, consider function $\mathit{count\_f}$ that counts
the number of times function $\mathit{g}$ uses its argument.
%
Function $\mathit{count\_f}$ can be defined as follows, using a local effect $\mathsf{Tick}$ (here, $\mathit{f}$ is supposed to be of type $  \forall   \rho  \ottsym{:}   \mathbf{Eff}    \ottsym{.}     \ottsym{(}   \ottnt{A}    \rightarrow_{ \rho }    \ottnt{B}   \ottsym{)}    \rightarrow_{ \rho }     \mathsf{Unit}   $).
%
\begin{flalign*}
   & \letdecl{\mathit{count\_f}}
  \Lambda  \rho  \ottsym{:}   \mathbf{Eff}   \ottsym{.}  \lambda  \mathit{g}  \ottsym{:}   \ottnt{A}    \rightarrow_{ \rho }    \ottnt{B}   \ottsym{.}   & \\ &    \quad    \quad   \ottkw{effect} \,  \mathsf{Tick}  ::  \ottsym{\{}  \mathsf{tick}  \ottsym{:}    \mathsf{Unit}    \Rightarrow    \mathsf{Unit}    \ottsym{\}}  \, \mathbf{in} \,  & \\ &    \quad    \quad    (   \mathbf{handle}_{ \mathsf{Tick} }  \,    \mathit{f} \, \ottsym{(}   \{  \mathsf{Tick}  \}  \,\underline{ \cup }\,  \rho   \ottsym{)} \,  (  \lambda  \mathit{x}  \ottsym{:}  \ottnt{A}  \ottsym{.}   \mathsf{tick} _{ \mathsf{Tick} }  \,  ()   \ottsym{;}  \mathit{g} \, \mathit{x}  )    & \\ &    \quad    \quad  \, \mathbf{with} \,  \ottsym{\{} \, \mathbf{return} \, \_  \mapsto  \lambda  \mathit{x}  \ottsym{:}   \mathsf{Int}   \ottsym{.}  \mathit{x}  \ottsym{\}}   \uplus   \ottsym{\{}  \mathsf{tick} \,  {}  \, \_ \, \mathit{k}  \mapsto  \lambda  \mathit{x}  \ottsym{:}   \mathsf{Int}   \ottsym{.}  \mathit{k} \,  ()  \,  (   \mathit{x}  +  1   )   \ottsym{\}}   )        \, 0
\end{flalign*}
%
In this program, we suppose that an effect algebra of sets allows exchanging non-parametric effect with any other effect and declare the label $\mathsf{Tick}$ locally within function $\mathit{count\_f}$.
%
If we declare $\mathsf{Tick}$ globally, the handler in $\mathit{count\_f}$ handles $\mathsf{tick}$
caused by application $\mathit{g} \, \mathit{x}$ against the programmer's will.

We have mainly two remaining works to extend {\lang} to local effects.
%
First, we must define a new syntax, typing rule, and reduction rule for local effects.
This work would be easy by following the prior work~\cite{biernacki_abstracting_2019}.
%
Secondly, we need to update the definition of effect algebras
because \citet{biernacki_abstracting_2019}'s equivalence relation on effects
depends on typing contexts.
% 
Thus, we must change the definition of equivalence $ \sim $ in effect algebras
to the one parameterized over typing contexts.
% 
We conjecture that there is no need to update safety conditions because
\citet{biernacki_abstracting_2019} use a scoped-rows-based representation and because
the only difference is the equivalence relation's dependency on typing contexts.

% it is required to check whether we need new safety conditions
% to prove the safety properties of the extended language.
% %
% \citet{biernacki_abstracting_2019} use an effect system with scoped rows,
% and the core equivalence rules over rows are the same as ours except for the one considering local effects.
% %
% Thus, we would need further investigation to give an effect algebra for local effects.
% %
% However, because equivalence on effects influences only effect algebras, we conjecture that
% the support for local effects does not require significant changes in our effect
% system itself, including the safety conditions.

\TY{The subsection about effect coercions is removed.}
% % 
% \subsection{Effect Coercions}
% % 
% \emph{Effect coercions}, introduced by \citet{biernacki_handle_2018, biernacki_abstracting_2019},
% explicitly change the order of labels in rows.
% %
% For example, using effect coercions,  we can also define the function $\mathit{count\_g}$ mentioned above, without local effects.
% \begin{flalign*}
%   \mathbf{let}\,\mathit{count\_g}
%     & = \Lambda \rho  \ottsym{:}   \mathbf{Eff}  . \lambda \mathit{g'}  \ottsym{:}   \ottnt{A}    \rightarrow_{ \rho }    \ottnt{B}  .                                                                                                                   & \\
%     & \qquad (\mathbf{handle}_{\mathsf{Tick}} \, \mathit{g}\,(\langle \mathsf{Tick} \mid \rho \rangle)\, (\lambda \mathit{x}  \ottsym{:}  \ottnt{A} . \mathsf{tick}\, ();\,[ \mathit{g'} \, \mathit{x} ]_{\mathsf{Tick}} ) & \\
%     & \qquad \mathbf{with} \{\mathbf{return}\, \_ \mapsto \lambda  \mathit{x}  \ottsym{:}   \mathsf{Int}   \ottsym{.}  \mathit{x} \} \uplus \{\mathsf{tick} \, \_ \, k \mapsto \lambda x : \mathsf{Int} . k\, ()\, (x + 1)\})\, 0     &
% \end{flalign*}
% %
% In this program, we use the syntax of scoped rows and suppose that $\mathsf{Tick}$ is declared globally.
% %
% We use a \emph{lift coercion} at $[ \mathit{g'} \, \mathit{x} ]_{\mathsf{Tick}}$.
% This coercion adds the label $\mathsf{Tick}$ to the top of row $\rho$.
% %
% Thus, the handler in $\mathit{count\_g}$ cannot handle $\mathsf{Tick}$ caused by evaluating $\mathit{g'} \, \mathit{x}$.

% In order to extend our language to effect coercions, we must extend the syntax
% and change the semantics to the one considering \emph{effect freeness}.
% %
% Effect freeness takes the form $n\textrm{-free}(\mathit{l}, \ottnt{E})$,
% which intuitively means that the n-th $\mathit{l}$ handler enclosing the evaluation context $\ottnt{E}$
% handles an $\mathit{l}$'s operation placed in the hole of $\ottnt{E}$.
% %
% The meaning of effect coercions is defined via effect freeness.
% %
% Changing the syntax and giving an instance reflecting effect coercions may be easy.
% %
% However, the change in the semantics can cause some difficulties in proving safety properties
% because we must consider the relationship between effect freeness and coercions in the abstract setting.
% %
% It is also unclear what safety conditions are adequate in the presence of effect coercions.

\OLD{
\subsection{Sets vs. Simple Rows}
We summarize the difference between effect systems with sets and simple rows.

First, we compare Example~\ref{exa:effset} and Example~\ref{exa:eff_simple_row}.
%
The main differences are the occurrences of effect variables and the label exchange rule.
%
The set instance allows effect variables to occur anywhere in effects,
but the simple row instance restricts effect variables at the end of rows.
This difference is trivial because we can easily create another instance of simple rows
that allows non-restricted occurrences of effect variables.
%
Unlike effect sets, simple rows have the label exchange rule whose one premise
compares $\ottnt{L_{{\mathrm{1}}}}$ and $\ottnt{L_{{\mathrm{2}}}}$. However, this premise is trivial because
the prohibited exchange, that is, the exchange of the same labels, is meaningless.
%
Therefore, there is no essential difference between effect sets and simple rows.

Secondly, we compare Example~\ref{exa:effset} and Example~\ref{exa:eff_simple_row_erasure}.
%
We describe how these differences appear in some settings.
%
When there are no parametric effects, the two instances are equal.
%
Since label names do not take parameters in this setting,
any label exchange is allowed, even in simple rows.
%
Furthermore, the choice of semantics does not cause differences
because the type-erasure semantics is the same as the non-type-erasure semantics in this setting.
%
When parametric effects exist, the type-erasure semantics causes the crucial difference, as seen in Section~\ref{sec:erasure}.
% 
Even in the non-type-erasure semantics, they are still different because of the label exchange rule in simple rows.
For example, $\mathbf{let} \, \_  \ottsym{=}   \mathsf{set} _{ \mathsf{State} \,  \mathsf{Int}  }  \,  {}  \, 0 \, \mathbf{in} \,  \mathsf{get} _{ \mathsf{State} \,  \mathsf{Bool}  }  \,  {}  \,  () $ is not well-typed under
the effect system with simple rows, but the one with sets accepts it.

\subsection{Qualified Simple Rows}\label{subsec:q_simple_rows}

The original effect system with simple rows \citep{hillerstrom_liberating_2016}
differs from the one we introduced in Example~\ref{exa:eff_simple_row} and Example~\ref{exa:eff_simple_row_erasure}
at the two points: prohibiting multiple labels and limiting instantiations of effect variables.
%
To distinguish them, we call what the effect system of \citet{hillerstrom_liberating_2016} is based on
\emph{qualified simple rows}.

An effect system with qualified simple rows realizes the features via its kind system shown below,
in the setting where there are no parametric effects.
%
\begin{mathpar}
  \inferrule{
  \Gamma \vdash P : \mathbf{Presence} \\
  \Gamma \vdash R : \mathbf{Row}_{\mathcal{L} \uplus \{l\} }
  }{
  \Gamma \vdash l : P ; R : \mathbf{Row}_{\mathcal{L}}
  }

  \inferrule{
    \Gamma \vdash R : \mathbf{Row}_{\emptyset}
  }{
    \Gamma \vdash \{ R \} : \mathbf{Eff}
  }
\end{mathpar}
%
$P$ is the presence with types $\mathsf{Pre}(A)$ or the absence $\mathsf{Abs}$.
$P = \mathsf{Pre}(A)$ represents that the row $l : P; R$ includes label $l$ typed as $A$.
$P = \mathsf{Abs}$ represents that the row $l : P; R$ does not include label $l$.
%
The set $\mathcal{L}$ attached to $\mathbf{Row}$ denotes the labels uncovered by the row.
%
If $\mathcal{L}$ is the empty set, then the row can be the effect.
%
Therefore, all effects do not have multiple labels.
%
Furthermore, the instantiation of row variables is limited by this kind system.
For example, consider the effect $\{l : \mathsf{Pre}(\ottnt{A}  \rightarrow  \ottnt{B}) ; \alpha\}$.
We cannot substitute rows that have the field $l$ for the row variable $\alpha$,
because the kind of $\alpha$ is $\mathbf{Row}_{\mathcal{L} \setminus \{l\}}$
where $\mathcal{L}$ is the whole set of labels.

To create an instance for qualified simple rows, we must extend {\lang}.
Specifically, we need to add \emph{qualified types} to limit substitutions for effect variables.
%
Adding qualified types makes an ARE of qualified simple rows more complex
because predicates in a context can be used.
For example, an ARE for qualified simple rows at least satisfies the following: if $\{l\} \not\!\!\olessthan \alpha$ is in $ \Delta $,
then $ \Delta  \vdash \{l\} \odot \alpha \sim \{l, \alpha\}$ holds.
%
However, attaching qualified types to {\lang} seemingly does not affect safety conditions.
% 
Thus, the extension of {\lang} to cover qualified simple rows does not seem complex.

\subsection{Local Effects}\label{subsec:local_eff}

\emph{Local effects} are algebraic effects declared locally \citep{biernacki_abstracting_2019, vilhena_type_2023}.
%
For example, we can define the function $\mathit{count\_g}$ that counts
the number of times $\mathit{g}$ uses its argument using a local effect $\mathsf{Tick}$,
where $\mathit{g}$ has the type $  \forall   \rho  \ottsym{:}   \mathbf{Eff}    \ottsym{.}     \ottsym{(}   \ottnt{A}    \rightarrow_{ \rho }    \ottnt{B}   \ottsym{)}    \rightarrow_{ \rho }     \mathsf{Unit}   $.
%
\begin{flalign*}
  \mathbf{let}\, \mathit{count\_g}
   & = \Lambda \rho  \ottsym{:}   \mathbf{Eff}  . \lambda \mathit{g'}  \ottsym{:}   \ottnt{A}    \rightarrow_{ \rho }    \ottnt{B}  .                                                                                                               & \\
   & \qquad \mathbf{effect}\,\mathsf{Tick} = \{ \mathsf{tick} : \mathsf{Unit} \Rightarrow \mathsf{Unit} \} \,\mathbf{in}                                                   & \\
   & \qquad (\mathbf{handle}_{\mathsf{Tick}} \, \mathit{g}\,([\mathsf{Tick}];\rho)\, (\lambda \mathit{x}  \ottsym{:}  \ottnt{A} . \mathsf{tick}\, ();\, \mathit{g'} \, \mathit{x} )                                   & \\
   & \qquad \mathbf{with} \{\mathbf{return}\, \_ \mapsto \lambda  \mathit{x}  \ottsym{:}   \mathsf{Int}   \ottsym{.}  \mathit{x} \} \uplus \{\mathsf{tick} \, \_ \, k \mapsto \lambda x : \mathsf{Int} . k\, ()\, (x + 1)\})\, 0 &
\end{flalign*}
%
In this program, we use the syntax of free rows and declare the local effect $\mathsf{Tick}$ at
$\mathbf{effect}\,\mathsf{Tick} = \{ \mathsf{tick} : \mathsf{Unit} \Rightarrow \mathsf{Unit} \} \,\mathbf{in}$.
%
If we declare $\mathsf{Tick}$ globally, the handler in $\mathit{coun\_g}$ handles $\mathsf{Tick}$
caused by evaluating $\mathit{g'} \, \mathit{x}$ against the programmer's will.
%

We have mainly two remaining works to extend {\lang} to local effects.
%
First, we must define a new syntax, typing rule, and reduction rule for local effects.
This work may be trivial, thanks to \citet{biernacki_abstracting_2019}.
%
Secondly, it is required to check whether we need new safety conditions
to prove the safety properties of the extended language.
%
\citet{biernacki_abstracting_2019} use an effect system with scoped rows,
and the core equivalence rules over rows are the same as ours except for the one considering local effects.
%
Because an instance, not a safety condition, gives such a new equivalence rule,
we conjecture there is no need to add safety conditions.

\subsection{Effect Coercions}
\emph{Effect coercions}, introduced by \citet{biernacki_handle_2018, biernacki_abstracting_2019},
explicitly change the order of labels in rows.
%
For example, using effect coercions,  we can also define the function $\mathit{count\_g}$ mentioned above.
\begin{flalign*}
  \mathbf{let}\,\mathit{count\_g}
   & = \Lambda \rho  \ottsym{:}   \mathbf{Eff}  . \lambda \mathit{g'}  \ottsym{:}   \ottnt{A}    \rightarrow_{ \rho }    \ottnt{B}  .                                                                                                                   & \\
   & \qquad (\mathbf{handle}_{\mathsf{Tick}} \, \mathit{g}\,(\langle \mathsf{Tick} \mid \rho \rangle)\, (\lambda \mathit{x}  \ottsym{:}  \ottnt{A} . \mathsf{tick}\, ();\,[ \mathit{g'} \, \mathit{x} ]_{\mathsf{Tick}} ) & \\
   & \qquad \mathbf{with} \{\mathbf{return}\, \_ \mapsto \lambda  \mathit{x}  \ottsym{:}   \mathsf{Int}   \ottsym{.}  \mathit{x} \} \uplus \{\mathsf{tick} \, \_ \, k \mapsto \lambda x : \mathsf{Int} . k\, ()\, (x + 1)\})\, 0     &
\end{flalign*}
%
In this program, we use the syntax of scoped rows and suppose that $\mathsf{Tick}$ is declared globally.
%
We use a \emph{lift coercion} at $[ \mathit{g'} \, \mathit{x} ]_{\mathsf{Tick}}$.
This coercion means adding the label $\mathsf{Tick}$ to the top of row $\rho$.
%
Thus, the handler in $\mathit{count\_g}$ cannot handle $\mathsf{Tick}$ caused by evaluating $\mathit{g'} \, \mathit{x}$.

In order to extend our language to effect coercions, we must extend the syntax
and change the semantics to the one using \emph{effect freeness}.
%
Effect freeness takes the form $n\textrm{-free}(\mathit{l}, \ottnt{E})$,
which intuitively means that the $n$-th $\mathit{l}$ handler enclosing the evaluation context $\ottnt{E}$
handles a $\mathit{l}$'s operation in the hole of $\ottnt{E}$.
%
Effect freeness has a close relationship with operational semantics and effect coercions.
%
Changing the syntax and giving an instance reflecting effect coercions may be easy.
%
However, the change in semantics can cause difficulty in proving safety properties
because we must consider the relationship between effect freeness and coercions in the abstract setting.
%
We must carefully check proofs and find new conditions to add to safety conditions.
}
